SalFBNet: Learning Pseudo-Saliency Distribution via Feedback Convolutional Networks

Feed-forward only convolutional neural networks (CNNs) may ignore intrinsic relationships and potential benefits of feedback connections in vision tasks such as saliency detection, despite their significant representation capabilities. In this work, we propose a feedback-recursive convolutional framework (SalFBNet) for saliency detection. The proposed feedback model can learn abundant contextual representations by bridging a recursive pathway from higher-level feature blocks to low-level layer. Moreover, we create a large-scale Pseudo-Saliency dataset to alleviate the problem of data deficiency in saliency detection. We first use the proposed feedback model to learn saliency distribution from pseudo-ground-truth. Afterwards, we fine-tune the feedback model on existing eye-fixation datasets. Furthermore, we present a novel Selective Fixation and Non-Fixation Error (sFNE) loss to make proposed feedback model better learn distinguishable eye-fixation-based features. Extensive experimental results show that our SalFBNet with fewer parameters achieves competitive results on the public saliency detection benchmarks, which demonstrate the effectiveness of proposed feedback model and Pseudo-Saliency data. Source codes and Pseudo-Saliency dataset can be found at https://github.com/gqding/SalFBNet

==> FBNet_Fig_fwfb_visualize.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.86\textwidth]{comp_fwfb.pdf}
    \caption{The visualization results of baseline forward-only model and feedback models on SALICON \cite{jiang2015salicon} validation set. FBNet \cite{ding2021fbnet} is our previous work.}
\label{fig:comp_fwfb}
\end{figure}

==> FBNet_Fig_pseudo_metrix.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.46\textwidth]{pseudo_cc.pdf}
    % \includegraphics[width=0.31\textwidth]{pseudo_sim.pdf}
    \includegraphics[width=0.46\textwidth]{pseudo_kldiv.pdf}\\
    \caption{Comparison of different model-annotators on Pseudo-Saliency dataset. The results are collected from annotators including MSINet \cite{kroner2020contextual}, DeepGaze \cite{linardos2021deepgaze}, EMLNet \cite{jia2020eml}, CASNet \cite{fan2018emotional}, and UNISAL \cite{droste2020unified}.}
\label{fig:pseudo-metrix}
\end{figure}

==> FBNet_Tab_fbfw_comp.tex <==
\begin{table}[!ht]
\centering \caption{Performance of baseline forward-only model and feedback models on SALICON \cite{jiang2015salicon} validation set.}
\resizebox{0.86\textwidth}{!}{
\begin{tabular}{  c | c  c  c  c  c  c  c }
\hline
\small Model     & \small AUC-J $\uparrow$ &  \small AUC-B $\uparrow$   &  \small  sAUC $\uparrow$   & \small  CC $\uparrow$ & \small  NSS $\uparrow$ & \small  KLdiv $\downarrow$ & \small  SIM $\uparrow$  \\
\hline\hline
\small Baseline\_Forward     & 0.8129  & 0.7509 & 0.6384 & 0.5564    & 1.1334  & 2.9065 & 0.5505   \\
\small \textbf{FBNet} \cite{ding2021fbnet}     & \textbf{0.9054}  & \textbf{0.8376} & \textbf{0.7151} & \textbf{0.7841}    & \textbf{1.6091}  & \textbf{0.8787} & \textbf{0.6900}     \\
\small \textbf{SalFBNet (our)}    & \textbf{0.8696}  & \textbf{0.8421} & \textbf{0.7331} & \textbf{0.8917}    & \textbf{1.9182}  & \textbf{0.2361} & \textbf{0.7684}   \\
\hline
\end{tabular}
}
\label{tab:feedback_forwad_comp}
\end{table}

==> FBNet_Tab_filtersize_comp.tex <==
\begin{table}[!t]
\centering \caption{$K$-folds performance of models with different filter sizes.}
\resizebox{0.86\textwidth}{!}{
\begin{tabular}{  c | c  c  c  c  c  c  c }
\hline
\small \#Filter Size              & \small AUC-J $\uparrow$ &  \small AUC-B $\uparrow$   &  \small  sAUC $\uparrow$   & \small  CC $\uparrow$ & \small  NSS $\uparrow$ & \small  KLdiv $\downarrow$ & \small  SIM $\uparrow$  \\
\hline\hline
\small 8 & 0.8365     & 0.8226  & 0.6881 & 0.7472 & 1.5337    & 0.6475  & 0.6559 \\
\small 16 & 0.8441     & 0.8304  & 0.6972 & 0.7749 & 1.5978    & 0.4953  & 0.6709 \\
\small 32 & 0.8485     & 0.8332  & 0.7064 & 0.7953 & 1.6551    & 0.4376  & 0.6851 \\
\small 64 & 0.8497     & 0.8359  & 0.7100 & 0.7992 & 1.6661    & 0.4324  & 0.6820 \\
\small 96 & 0.8501     & 0.8350  & 0.7084 & \textbf{0.8040} & 1.6787    & 0.4286  & 0.6820 \\
\small 128 & \textbf{0.8507}     & \textbf{0.8362}  & 0.7116 & 0.8039 & \textbf{1.6791}    & \textbf{0.4008}  & \textbf{0.6872} \\
\small 160 & 0.8500     & 0.8357  & \textbf{0.7131} & 0.8002 & 1.6743    & 0.4038  & 0.6815 \\
\small 196 & 0.8503     & 0.8361  & 0.7114 & 0.8025 & 1.6781    & 0.4167  & 0.6824 \\
\hline
\end{tabular}
}
\label{tab:filtersize_comp}
\end{table}

==> FBNet_Tab_pseudosaliency_comp_backbones.tex <==
\begin{table*}[!t]
\centering \caption{Comparison of pre-trained performance of feedback models with different backbones and initialization strategies. \textbf{ImageNet} and \textbf{Random} denote the model parameters are initialized from ImageNet \cite{krizhevsky2012imagenet} pre-trained weights and random initialized weights. \textbf{Init.} means the initialization of the model, \textbf{Eval.} means the evaluation set.}
\resizebox{\textwidth}{!}{
\begin{tabular}{  c | c | c | c | c | c  c  c  c  c  c  c }
\hline
% \small Dataset  &  \multicolumn{8}{c}{SALICON \cite{jiang2015salicon} validation set}   \\
% \hline
\small Backbone & \#Params (M)  &  Init.  & Train & Eval.  & \small AUC-J $\uparrow$ &  \small AUC-B $\uparrow$   &  \small  sAUC $\uparrow$   & \small  CC $\uparrow$ & \small  NSS $\uparrow$ & \small  KLdiv $\downarrow$ & \small  SIM $\uparrow$  \\
\hline\hline
\small Densenet121 & 24.80 & ImageNet    & Pseudo-Saliency  & SALICON  & 0.8639  & 0.8291 & 0.7147 & 0.8663    & 1.8626  & 0.3687 & 0.7457   \\
\small ResNet18    & 17.26    & ImageNet    & Pseudo-Saliency & SALICON   & 0.8685  & 0.8334 & 0.7214 & 0.8863    & 1.9162  & 0.2769 & 0.7659     \\
\small ResNet50 & 28.18  & ImageNet    & Pseudo-Saliency & SALICON   & 0.8674  & 0.8343 & 0.7202 & 0.8812    & 1.9011  & 0.2900 & 0.7588   \\
\small VGG16 & 23.64 & ImageNet    & Pseudo-Saliency & SALICON  & 0.8641  & 0.8437 & 0.7237 & 0.8661    & 1.8355  & 0.2955 & 0.7354    \\
\hline
\small Densenet121 & 24.80  & Random    & Pseudo-Saliency & SALICON  & 0.8650  & 0.8325 & 0.7160 & 0.8714    & 1.8690  & 0.3507 & 0.7580  \\
\small ResNet18   & 17.26     & Random   & Pseudo-Saliency & SALICON   & 0.8680  & 0.8329 & 0.7209 & 0.8843    & 1.9106  & 0.2812 & 0.7674  \\
\small ResNet50  & 28.18 & Random   & Pseudo-Saliency & SALICON   & 0.8673  & 0.8341 & 0.7209 & 0.8812    & 1.9011  & 0.2887 & 0.7585 \\
\small VGG16  & 23.64 & Random   & Pseudo-Saliency & SALICON   & 0.8608  & 0.8371 & 0.7128 & 0.8500    & 1.7898  & 0.3026 & 0.7296   \\
\hline
\small FBNet-Fixed64 \cite{ding2021fbnet}   & 1.18 & Random   & Pseudo-Saliency & SALICON   & 0.8597  & 0.8374 & 0.7114 & 0.8445    & 1.7855  & 0.3156 & 0.7214  \\
\small FBNet-Fixed128 \cite{ding2021fbnet}  & 5.32 & Random    & Pseudo-Saliency & SALICON  & 0.8599  & 0.8375 & 0.7108 & 0.8464    & 1.7829  & 0.3134 & 0.7194  \\
\small Res18Fixed128 & 5.97   & Random    & Pseudo-Saliency & SALICON  & 0.8681  & 0.8336 & 0.7211 & 0.8847    & 1.9123  & 0.2647 & 0.7616  \\
\hline
\end{tabular}
}
\label{tab:pseoudo_comp_backbones}
\end{table*}
